Does the Goal Matter? Emotion Recognition Tasks Can Change the Social Value of Facial Mimicry towards Artificial Agents

In this paper, we present a study aimed at understanding whether the embodiment and humanlikeness of an artificial agent can affect people's spontaneous and instructed mimicry of its facial expressions. The study followed a mixed experimental design and revolved around an emotion recognition task. Participants were randomly assigned to one level of humanlikeness (between-subject variable: humanlike, characterlike, or morph facial texture of the artificial agents) and observed the facial expressions displayed by a human (control) and three artificial agents differing in embodiment (within-subject variable: video-recorded robot, physical robot, and virtual agent). To study both spontaneous and instructed facial mimicry, we divided the experimental sessions into two phases. In the first phase, we asked participants to observe and recognize the emotions displayed by the agents. In the second phase, we asked them to look at the agents' facial expressions, replicate their dynamics as closely as possible, and then identify the observed emotions. In both cases, we assessed participants' facial expressions with an automated Action Unit (AU) intensity detector. Contrary to our hypotheses, our results disclose that the agent that was perceived as the least uncanny, and most anthropomorphic, likable, and co-present, was the one spontaneously mimicked the least. Moreover, they show that instructed facial mimicry negatively predicts spontaneous facial mimicry. Further exploratory analyses revealed that spontaneous facial mimicry appeared when participants were less certain of the emotion they recognized. Hence, we postulate that an emotion recognition goal can flip the social value of facial mimicry as it transforms a likable artificial agent into a distractor.

==> refs.tex <==
@article{ruch2013,
  title={Investigating facial features of four types of laughter in historic illustrations},
  author={Ruch, Willibald Friedrich and Hofmann, Jennifer and Platt, Tracey},
  journal={European Journal of Humour Research},
  volume={1},
  number={1},
  pages={99--118},
  year={2013}
}

@inproceedings{XiongD13, 
    author = {Xuehan Xiong and Fernando {De la Torre}}, 
    title = {Supervised Descent Method and its Applications to Face Alignment}, 
    booktitle = {IEEE Conference on Computer Vision and Pattern Recognition}, 
    year = {2013} 
} 

@book{hall_hidden_1969,
	title = {{The Hidden Dimension}},
	volume = {1990},
	publisher = {Anchor Books New York},
	author = {Hall, E. T.},
	year = {1969},
}

@incollection{piana2013automated,
  title={Automated analysis of non-verbal expressive gesture},
  author={Piana, S and Mancini, M and Camurri, A and Varni, G and Volpe, G},
  booktitle={Human Aspects in Ambient Intelligence},
  pages={41--54},
  year={2013},
  publisher={Atlantis Press}
}



@incollection{Ruch_epxressive2001,
  author      = "Ruch, W. and Ekman, P.",
  title       = "The expressive patterns of laughter",
  editor      = "Kaszniak, A.",
  booktitle   = "Emotion, Qualia and Consciousness",
  publisher   = "World Scientific",
  pages       = "426--443",
  year        = 2001
}

@inproceedings{XD13,
  title={Supervised descent method and its applications to face alignment},
  author={Xiong, Xuehan and Torre, Fernando},
  booktitle={IEEE Conference on Computer Vision and Pattern Recognition},
  pages={532--539},
  year={2013}
}

@article{ruch2008gelotophobic,
  title={Who is gelotophobic? Assessment criteria for the fear of being laughed at},
  author={Ruch, Willibald and Proyer, Ren{\'e} T},
  journal={Swiss Journal of Psychology},
  volume={67},
  number={1},
  pages={19--27},
  year={2008},
  publisher={Verlag Hans Huber}
}

@article{gosling2003very,
  title={A very brief measure of the Big-Five personality domains},
  author={Gosling, Samuel D and Rentfrow, Peter J and Swann, William B},
  journal={Journal of Research in Personality},
  volume={37},
  number={6},
  pages={504--528},
  year={2003}
}

@article{rosenthal2014design,
  title={How design characteristics of robots determine evaluation and uncanny valley related responses},
  author={Rosenthal-von der P{\"u}tten, Astrid M and Kr{\"a}mer, Nicole C},
  journal={Computers in Human Behavior},
  volume={36},
  pages={422--439},
  year={2014}
}

@article{bartneck2009measurement,
  title={Measurement instruments for the anthropomorphism, animacy, likeability, perceived intelligence, and perceived safety of robots},
  author={Bartneck, Christoph and Kuli{\'c}, Dana and Croft, Elizabeth and Zoghbi, Susana},
  journal={Int. Journal of Social Robotics},
  volume={1},
  number={1},
  pages={71--81},
  year={2009}
}

@article{walters2008avoiding,
  title={Avoiding the uncanny valley: robot appearance, personality and consistency of behavior in an attention-seeking home scenario for a robot companion},
  author={Walters, Michael L and Syrdal, Dag S and Dautenhahn, Kerstin and Te Boekhorst, Ren{\'e} and Koay, Kheng Lee},
  journal={Autonomous Robots},
  volume={24},
  number={2},
  pages={159--178},
  year={2008}
}

@article{mcdonnell2012render,
  title={Render me real?: investigating the effect of render style on the perception of animated virtual humans},
  author={McDonnell, Rachel and Breidt, Martin and B{\"u}lthoff, Heinrich H},
  journal={ACM Trans. on Graphics},
  volume={31},
  number={4},
  pages={91},
  year={2012}
}

@inproceedings{paetzel:icsr,
   title = {{Congruency matters - How ambiguous gender
cues increase a robot's uncanniness}},
   author = {Paetzel, Maike and Peters, Christopher and Nystr\"{o}m, Ingela and Castellano, Ginevra},
   year =       "2016",
   booktitle  = "International Conference on Social Robotics",
}

@misc{FaceGen,
  title = {{FaceGen Modeller}},
  howpublished = {\url{http://facegen.com/}},
  note = {Accessed: 2018-04-10}
}

@misc{CereProc,
  title = {{CereProc}},
  howpublished = {\url{https://www.cereproc.com/}},
  note = {Accessed: 2016-05-08}
}

@incollection{almoubayed2012furhat,
  title={{Furhat: a back-projected human-like robot head for multiparty human-machine interaction}},
  author={Al Moubayed, Samer and Beskow, Jonas and Skantze, Gabriel and Granstr{\"o}m, Bj{\"o}rn},
  booktitle={Cognitive Behavioural Systems},
  pages={114--130},
  year={2012}
}

@article{katsyri2015review,
  title={A review of empirical evidence on different uncanny valley hypotheses: support for perceptual mismatch as one road to the valley of eeriness},
  author={K{\"a}tsyri, Jari and F{\"o}rger, Klaus and M{\"a}k{\"a}r{\"a}inen, Meeri and Takala, Tapio},
  journal={Frontiers in Psychology},
  volume={6},
  year={2015}
}

@book{royle2003uncanny,
  title={The uncanny},
  author={Royle, Nicholas},
  year={2003},
  publisher={Manchester University Press}
}


@inproceedings{gratch2006virtual,
  title={Virtual rapport},
  author={Gratch, Jonathan and Okhmatovskaia, Anna and Lamothe, Francois and Marsella, Stacy and Morales, Mathieu and van der Werf, Rick J and Morency, Louis-Philippe},
  booktitle={Int. Workshop on Intelligent Virtual Agents},
  pages={14--27},
  year={2006}
}

@article{riek2010my,
  title={When my robot smiles at me: Enabling human-robot rapport via real-time head gesture mimicry},
  author={Riek, Laurel D and Paul, Philip C and Robinson, Peter},
  journal={Journal on Multimodal User Interfaces},
  volume={3},
  number={1-2},
  pages={99--108},
  year={2010}
}

@inproceedings{fuente2015influence,
  title={Influence of Upper Body Pose Mirroring in Human-Robot Interaction},
  author={Fuente, Luis A and Ierardi, Hannah and Pilling, Michael and Crook, Nigel T},
  booktitle={Int. Conference on Social Robotics},
  pages={214--223},
  year={2015}
}

@article{lakin2003chameleon,
  title={The chameleon effect as social glue: Evidence for the evolutionary significance of nonconscious mimicry},
  author={Lakin, Jessica L and Jefferis, Valerie E and Cheng, Clara Michelle and Chartrand, Tanya L},
  journal={Journal of Nonverbal Behavior},
  volume={27},
  number={3},
  pages={145--162},
  year={2003}
}

@book{keysers2011empathic,
  title={The empathic brain: How the discovery of mirror neurons changes our understanding of human nature},
  author={Keysers, Christian},
  year={2011},
  publisher={CreateSpace Independent Publishing Platform}
}

@book{tinwell2014uncanny,
  title={The Uncanny Valley in Games and Animation},
  author={Tinwell, Angela},
  year={2014},
  publisher={CRC Press}
}

@article{stel2010mimicry,
  title={Mimicry in social interaction: Benefits for mimickers, mimickees, and their interaction},
  author={Stel, Mari{\"e}lle and Vonk, Roos},
  journal={British Journal of Psychology},
  volume={101},
  number={2},
  pages={311--323},
  year={2010}
}

@article{havas2010cosmetic,
  title={Cosmetic use of botulinum toxin-A affects processing of emotional language},
  author={Havas, David A and Glenberg, Arthur M and Gutowski, Karol A and Lucarelli, Mark J and Davidson, Richard J},
  journal={Psychological Science},
  year={2010},
  publisher={Sage Publications}
}

@article{likowski2008modulation,
  title={Modulation of facial mimicry by attitudes},
  author={Likowski, Katja U and M{\"u}hlberger, Andreas and Seibt, Beate and Pauli, Paul and Weyers, Peter},
  journal={Journal of Experimental Social Psychology},
  volume={44},
  number={4},
  pages={1065--1072},
  year={2008}
}

@article{hofree2014bridging,
  title={Bridging the mechanical and the human mind: spontaneous mimicry of a physically present android},
  author={Hofree, Galit and Ruvolo, Paul and Bartlett, Marian Stewart and Winkielman, Piotr},
  journal={PloS one},
  volume={9},
  number={7},
  year={2014}
}

@article{mori2012uncanny,
  title={The uncanny valley [from the field]},
  author={Mori, Masahiro and MacDorman, Karl F and Kageki, Norri},
  journal={IEEE Robotics \& Automation Magazine},
  volume={19},
  number={2},
  pages={98--100},
  year={2012}
}

@incollection{chapman83,
  title={{Humor and laughter in social interaction
and some implications for humor research}},
  author={Chapman, A.},
  booktitle={Handbook of Humor Research},
volume ={1},
editor={McGhee, P. and Goldstein, J.},
  pages={135--157},
  year={1983}
}

@article{ho2010revisiting,
  title={Revisiting the uncanny valley theory: Developing and validating an alternative to the Godspeed indices},
  author={Ho, Chin-Chang and MacDorman, Karl F},
  journal={Computers in Human Behavior},
  volume={26},
  number={6},
  pages={1508--1518},
  year={2010}
}

@inproceedings{vlachos2002,
  title={Non-linear dimensionality reduction techniques for classification and visualization},
  author={Vlachos, Michail and Domeniconi, Carlotta and Gunopulos, Dimitrios and Kollios, George and Koudas, Nick},
  booktitle={ACM International Conference on Knowledge Discovery and Data Mining},
  pages={645--651},
  year={2002}
}

@article{pedregosa2011,
 title={Scikit-learn: Machine Learning in {P}ython},
 author={Pedregosa, F. and Varoquaux, G. and Gramfort, A. and Michel, V.
         and Thirion, B. and Grisel, O. and Blondel, M. and Prettenhofer, P.
         and Weiss, R. and Dubourg, V. and Vanderplas, J. and Passos, A. and
         Cournapeau, D. and Brucher, M. and Perrot, M. and Duchesnay, E.},
 journal={Journal of Machine Learning Research},
 volume={12},
 pages={2825--2830},
 year={2011}
}

@article{provine2004laughing,
  title={Laughing, tickling, and the evolution of speech and self},
  author={Provine, Robert R},
  journal={Current Directions in Psychological Science},
  volume={13},
  number={6},
  pages={215--218},
  year={2004}
}

@article{grammer1990ritualisation,
  title={The ritualisation of laughter},
  author={Grammer, Karl and Eibl-Eibesfeldt, Irenaus},
  journal={Nat{\"u}rlichkeit der Sprache und der Kultur},
  volume={18},
  pages={192--214},
  year={1990},
  publisher={Universit{\"a}tsverlag Dr. Norbert Brockmeyer Bochum,, Germany}
}

@inproceedings{niewiadomski2012towards,
  title={Towards multimodal expression of laughter},
  author={Niewiadomski, Rados{\l}aw and Pelachaud, Catherine},
  booktitle={Int. Conference on Intelligent Virtual Agents},
  pages={231--244},
  year={2012}
}

@inproceedings{urbain2013evaluation,
  title={{Evaluation of HMM-based laughter synthesis}},
  author={Urbain, J{\'e}r{\^o}me and Cakmak, H{\"u}seyin and Dutoit, Thierry},
  booktitle={IEEE Int. Conference on Acoustics, Speech and Signal Processing},
  pages={7835--7839},
  year={2013}
}

@inproceedings{becker2009laughter,
  title={Laughter in social robotics-no laughing matter},
  author={Becker-Asano, Christian and Ishiguro, Hiroshi},
  booktitle={Int. Workshop on Social Intelligence Design},
  pages={287--300},
  year={2009}
}

@InProceedings{Mirnig2016,
author="Mirnig, Nicole and Stadler, Susanne and Stollnberger, Gerald and Giuliani, Manuel and Tscheligi, Manfred",
title="Robot Humor: How Self-Irony and Schadenfreude Influence People{'}s Rating of Robot Likability",
booktitle="IEEE Int. Symposium on Robot and Human Interactive Communication",
year="2016"
}

@article{EF02,
  title={Facial {A}ction {C}oding {S}ystem},
  author={Hager, Joseph C and Ekman, Paul and Friesen, Wallace V},
  journal={Salt Lake City, UT: A Human Face},
  year={2002}
}

@incollection{adams2011android,
  title={An android head for social-emotional intervention for children with autism spectrum conditions},
  author={Adams, Andra and Robinson, Peter},
  booktitle={Affective Computing and Intelligent Interaction},
  pages={183--190},
  year={2011}
}

@article{kulesza2015face,
  title={The face of the chameleon: The experience of facial mimicry for the mimicker and the mimickee},
  author={Kulesza, Wojciech Marek and Cis{\l}ak, Aleksandra and Vallacher, Robin R and Nowak, Andrzej and Czekiel, Martyna and Bedynska, Sylwia},
  journal={The Journal of Social Psychology},
  volume={155},
  number={6},
  pages={590--604},
  year={2015}
}

@article{stel2008facial,
  title={Facial feedback mechanisms in autistic spectrum disorders},
  author={Stel, Mari{\"e}lle and van den Heuvel, Claudia and Smeets, Raymond C},
  journal={Journal of Autism and Developmental Disorders},
  volume={38},
  number={7},
  pages={1250--1258},
  year={2008}
}

@inproceedings{pecune2015laughing,
  title={Laughing with a virtual agent},
  author={Pecune, Florian and Mancini, Maurizio and Biancardi, Beatrice and Varni, Giovanna and Ding, Yu and Pelachaud, Catherine and Volpe, Gualtiero and Camurri, Antonio},
  booktitle={Proceedings of the 2015 International Conference on Autonomous Agents and Multiagent Systems},
  pages={1817--1818},
  year={2015},
  organization={Int. Foundation for Autonomous Agents and Multiagent Systems}
}


@inproceedings{griffin2015gesture,
  title={Gesture mimicry in expression of laughter},
  author={Griffin, Harry and Varni, Giovanna and Volpe, Gualtiero and Lourido, Gisela Tom{\'e} and Mancini, Maurizio and Bianchi-Berthouze, Nadia},
  booktitle={Int. Conference on Affective Computing and Intelligent Interaction },
  pages={677--683},
  year={2015}
}

@inproceedings{leyzberg2012physical,
  title={The physical presence of a robot tutor increases cognitive learning gains},
  author={Leyzberg, Daniel and Spaulding, Samuel and Toneva, Mariya and Scassellati, Brian},
  year={2012},
  booktitle={CogSci}
}

@article{bourgeois2008impact,
  title={The impact of social context on mimicry},
  author={Bourgeois, Patrick and Hess, Ursula},
  journal={Biological Psychology},
  volume={77},
  number={3},
  pages={343--352},
  year={2008}
}

@article{tapus2007grand,
  title={The grand challenges in socially assistive robotics.},
  author={Tapus, A and Mataric, MJ and Scassellati, B},
  year={2007},
  journal={ Robotics and Automation Magazine},
  volume={14},
  number={1},
  pages={1-7}
}


@article{boucenna2016,
  title={Robots learn to recognize individuals from imitative encounters with people and avatars},
  author={Boucenna, Sofiane and Cohen, David and Meltzoff, Andrew N and Gaussier, Philippe and Chetouani, Mohamed},
  journal={Scientific Reports},
  volume={6},
  year={2016}
}



@article{hess2013,
  title={Emotional mimicry as social regulation},
  author={Hess, Ursula and Fischer, Agneta},
  journal={Personality and Social Psychology Review},
  volume={17},
  number={2},
  pages={142--157},
  year={2013},
  publisher={Sage Publications}
}

@article{hess2014,
  title={Emotional mimicry: Why and when we mimic emotions},
  journal={Social and Personality Psychology Compass},
  author={Hess, Ursula and Fischer, Agneta},
  volume={8},
  number={2},
  pages={45--57},
  year={2014}
}

@article{dumas2010,
  title={Inter-brain synchronization during social interaction},
  author={Dumas, Guillaume and Nadel, Jacqueline and Soussignan, Robert and Martinerie, Jacques and Garnero, Line},
  journal={PloS One},
  volume={5},
  number={8},
  year={2010}
}

@article{brothers1990,
  title={The neural basis of primate social communication},
  author={Brothers, Leslie},
  journal={Motivation and emotion},
  volume={14},
  number={2},
  pages={81--91},
  year={1990}
}

@article{dunbar2008,
  title={Mind the gap: or why humans aren't just great apes},
  author={Dunbar, RIM},
  year={2008}
}


@article{Marwan07,
title = "Recurrence plots for the analysis of complex systems",
journal = "Physics Reports",
volume = "438",
number = "5–6",
pages = "237 - 329",
year = "2007",
author = "Norbert Marwan and M. Carmen Romano and Marco Thiel and Jürgen Kurths",
}

@article{fasola2013socially,
  title={A socially assistive robot exercise coach for the elderly},
  author={Fasola, Juan and Mataric, Maja},
  journal={Journal of Human-Robot Interaction},
  volume={2},
  number={2},
  pages={3--32},
  year={2013}
}

@article{bennett2014deriving,
  title={Deriving minimal features for human-like facial expressions in robotic faces},
  author={Bennett, Casey C and {\v{S}}abanovi{\'c}, Selma},
  journal={Int. Journal of Social Robotics},
  volume={6},
  number={3},
  pages={367--381},
  year={2014}
}

@inproceedings{moosaei2017using,
  title={Using Facially Expressive Robots to Calibrate Clinical Pain Perception},
  author={Moosaei, Maryam and Das, Sumit K and Popa, Dan O and Riek, Laurel D},
  booktitle={ACM/IEEE Int. Conference on Human-Robot Interaction},
  pages={32--41},
  year={2017}
}


@article{serra2009,
  title={Cross recurrence quantification for cover song identification},
  author={Serra, Joan and Serra, Xavier and Andrzejak, Ralph G},
  journal={New Journal of Physics},
  volume={11},
  number={9},
  year={2009}
}

@article{Boucenna2016,
	Author = {Boucenna, S. and Cohen D. and Gaussier, P. and Meltzoff, A N and Chetouani, M.},
	Date-Added = {2015-12-12 21:44:36 +0000},
	Date-Modified = {2016-01-31 19:10:04 +0000},
	Journal = {Scientific Reports},
	Title = {Robots Learn to Recognize Individuals from Imitative Encounters with People and Avatars},
	Year = {2016}
}


@inproceedings{varni2015,
  title={SyncPy: a unified open-source analytic library for synchrony},
  author={Varni, Giovanna and Avril, Marie and Usta, Adem and Chetouani, Mohamed},
  booktitle={Workshop on Modeling INTERPERsonal SynchrONy And infLuence},
  pages={41--47},
  year={2015}
}

@book{ekman1997face,
  title={What the face reveals: Basic and applied studies of spontaneous expression using the Facial Action Coding System (FACS)},
  author={Ekman, Paul and Rosenberg, Erika L},
  year={1997},
  publisher={Oxford University Press, USA}
}

@article{rammstedt2007measuring,
  title={Measuring personality in one minute or less: A 10-item short version of the Big Five Inventory in English and German},
  author={Rammstedt, Beatrice and John, Oliver P},
  journal={Journal of Research in Personality},
  volume={41},
  number={1},
  pages={203--212},
  year={2007}
}

@book{davis1980interpersonal,
  title={Interpersonal reactivity index},
  author={Davis, Mark H},
  year={1980},
  publisher={Edwin Mellen Press}
}

@article{harms2004internal,
  title={Internal consistency and reliability of the networked minds measure of social presence},
  author={Harms, Chad and Biocca, Frank},
  year={2004}
}

@article{breazeal2003emotion,
  title={Emotion and sociable humanoid robots},
  author={Breazeal, Cynthia},
  journal={Int. Journal of Human-Computer Studies},
  volume={59},
  number={1-2},
  pages={119--155},
  year={2003}
}

@inproceedings{beer2009emotion,
  title={Emotion recognition of virtual agents facial expressions: the effects of age and emotion intensity},
  author={Beer, Jenay M and Fisk, Arthur D and Rogers, Wendy A},
  booktitle={Human Factors and Ergonomics Society Annual Meeting},
  volume={53},
  number={2},
  pages={131--135},
  year={2009}
}

@inproceedings{aifanti2010mug,
  title={{The MUG facial expression database}},
  author={Aifanti, Niki and Papachristou, Christos and Delopoulos, Anastasios},
  booktitle={IEEE Int. Workshop on Image Analysis for Multimedia Interactive Services},
  pages={1--4},
  year={2010}
}

@article{kirby2010affective,
  title={Affective social robots},
  author={Kirby, Rachel and Forlizzi, Jodi and Simmons, Reid},
  journal={Robotics and Autonomous Systems},
  volume={58},
  number={3},
  pages={322--332},
  year={2010}
}

@article{leite2013social,
  title={Social robots for long-term interaction: a survey},
  author={Leite, Iolanda and Martinho, Carlos and Paiva, Ana},
  journal={Int. Journal of Social Robotics},
  volume={5},
  number={2},
  pages={291--308},
  year={2013}
}

@inproceedings{disalvo2002all,
  title={All robots are not created equal: the design and perception of humanoid robot heads},
  author={DiSalvo, Carl F and Gemperle, Francine and Forlizzi, Jodi and Kiesler, Sara},
  booktitle={Conference on Designing Interactive Systems: Processes, Practices, Methods, and Techniques},
  pages={321--326},
  year={2002}
}

@article{vinciarelli2014survey,
  title={A survey of personality computing},
  author={Vinciarelli, Alessandro and Mohammadi, Gelareh},
  journal={IEEE Trans. on Affective Computing},
  volume={5},
  number={3},
  pages={273--291},
  year={2014}
}

@book{brunswik1956perception,
  title={Perception and the representative design of psychological experiments},
  author={Brunswik, Egon},
  year={1956},
  publisher={Univ of California Press}
}

@article{li2015benefit,
  title={The benefit of being physically present: A survey of experimental works comparing copresent robots, telepresent robots and virtual agents},
  author={Li, Jamy},
  journal={Int. Journal of Human-Computer Studies},
  volume={77},
  pages={23--37},
  year={2015}
}

@article{lee2006physically,
  title={Are physically embodied social agents better than disembodied social agents?: The effects of physical embodiment, tactile interaction, and people's loneliness in human--robot interaction},
  author={Lee, Kwan Min and Jung, Younbo and Kim, Jaywoo and Kim, Sang Ryong},
  journal={Int. Journal of Human-Computer Studies},
  volume={64},
  number={10},
  pages={962--973},
  year={2006}
}

@inproceedings{thellman2016physical,
  title={Physical vs. Virtual agent embodiment and effects on social interaction},
  author={Thellman, Sam and Silvervarg, Annika and Gulz, Agneta and Ziemke, Tom},
  booktitle={Int. Conference on Intelligent Virtual Agents},
  pages={412--415},
  year={2016}
}

@article{gifford1994lens,
  title={A lens-mapping framework for understanding the encoding and decoding of interpersonal dispositions in nonverbal behavior.},
  author={Gifford, Robert},
  journal={J. of Personality and Social Psychology},
  volume={66},
  number={2},
  pages={398},
  year={1994},
  publisher={American Psychological Association}
}

@article{gratch2005lessons,
  title={Lessons from emotion psychology for the design of lifelike characters},
  author={Gratch, Jonathan and Marsella, Stacy},
  journal={Applied Artificial Intelligence},
  volume={19},
  number={3-4},
  pages={215--233},
  year={2005}
}

@inproceedings{nass1994computers,
  title={Computers are social actors},
  author={Nass, Clifford and Steuer, Jonathan and Tauber, Ellen R},
  booktitle={SIGCHI Conference on Human Factors in Computing Systems},
  pages={72--78},
  year={1994}
}

@book{kirlik2006adaptive,
  title={Adaptive perspectives on human-technology interaction: Methods and models for cognitive engineering and human-computer interaction},
  author={Kirlik, Alex},
  year={2006},
  publisher={Oxford University Press}
}

@inproceedings{riek2009anthropomorphism,
  title={How anthropomorphism affects empathy toward robots},
  author={Riek, Laurel D and Rabinowitch, Tal-Chen and Chakrabarti, Bhismadev and Robinson, Peter},
  booktitle={ACM/IEEE Int. Conference on Human Robot Interaction},
  pages={245--246},
  year={2009}
}

@article{tinwell2011facial,
  title={Facial expression of emotion and perception of the Uncanny Valley in virtual characters},
  author={Tinwell, Angela and Grimshaw, Mark and Nabi, Debbie Abdel and Williams, Andrew},
  journal={Computers in Human Behavior},
  volume={27},
  number={2},
  pages={741--749},
  year={2011}
}

@inproceedings{becker2011evaluating,
  title={Evaluating facial displays of emotion for the android robot Geminoid F},
  author={Becker-Asano, Christian and Ishiguro, Hiroshi},
  booktitle={IEEE Workshop on Affective Computational Intelligence},
  pages={1--8},
  year={2011}
}

@inproceedings{hortensius2017perception,
  title={The perception of emotion in artificial agents},
  author={Hortensius, Ruud and Hekele, Felix and Cross, Emily S},
  year={2017},
  booktitle={PsyArXiv}
}

@article{lazzeri2015can,
  title={Can a humanoid face be expressive? A psychophysiological investigation},
  author={Lazzeri, Nicole and Mazzei, Daniele and Greco, Alberto and Rotesi, Annalisa and Lanat{\`a}, Antonio and De Rossi, Danilo Emilio},
  journal={Frontiers in Bioengineering and Biotechnology},
  volume={3},
  pages={64},
  year={2015}
}

@article{macdorman2015individual,
  title={Individual differences predict sensitivity to the uncanny valley},
  author={MacDorman, Karl F and Entezari, Steven O},
  journal={Interaction Studies},
  volume={16},
  number={2},
  pages={141--172},
  year={2015}
}

@article{chaby2017gaze,
  title={Gaze behavior consistency among older and younger adults when looking at emotional faces},
  author={Chaby, Laurence and Hupont, Isabelle and Avril, Marie and Luherne-du Boullay, Viviane and Chetouani, Mohamed},
  journal={Frontiers in Psychology},
  volume={8},
  pages={548},
  year={2017}
}

@inproceedings{chevalier:hal-01203702,
TITLE = {{Impact of Personality on the Recognition of Emotion Expressed via Human, Virtual, and Robotic Embodiments}},
AUTHOR = {Chevalier, Pauline and Martin, Jean-Claude and Isableu, Brice and Tapus, Adriana},
BOOKTITLE = {{IEEE RO-MAN}},
YEAR = {2015}
} 

@article{canli2002neuroimaging,
title={Neuroimaging of emotion and personality: Scientific evidence and ethical considerations},
author={Canli, Turhan and Amin, Zenab},
journal={Brain and Cognition},
volume={50},
number={3},
pages={414--431},
year={2002}
} 

@inproceedings{skantze2012iristk,
  title={{IrisTK: a Statechart-based Toolkit for Multi-party Face-to-face Interaction}},
  author={Skantze, Gabriel and Al Moubayed, Samer},
  booktitle={Int. Conference on Multimodal Interaction},
  pages={69--76},
  year={2012}
}

@article{komulainen2014effect,
title={The effect of personality on daily life emotional processes},
author={Komulainen, Emma and Meskanen, Katarina and Lipsanen, Jari and Lahti, Jari Marko and Jylh{\"a}, Pekka and Melartin, Tarja and Wichers, Marieke and Isomets{\"a}, Erkki and Ekelund, Jesper},
journal={PLoS One},
volume={9},
number={10},
year={2014}
} 

@article{davis1980multidimensional,
  title={A multidimensional approach to individual differences in empathy},
  author={Davis, Mark H and others},
  year={1980},
  journal={JSAS Catalog of Selected Documents in Psychology}
}

@article{becker2007confounded,
  title={The confounded nature of angry men and happy women},
  author={Becker, D Vaughn and Kenrick, Douglas T and Neuberg, Steven L and Blackwell, KC and Smith, Dylan M},
  journal={J. of Personality and Social Psychology},
  volume={92},
  number={2},
  pages={179},
  year={2007}
}

@article{vinciarelli2015,
  title={New social signals in a new interaction world: the next frontier for social signal processing},
  author={Vinciarelli, Alessandro and Pentland, Alex},
  journal={IEEE Systems, Man, and Cybernetics Magazine},
  volume={1},
  number={2},
  pages={10--17},
  year={2015}
}


@inproceedings{seo2015,
  title={Poor thing! would you feel sorry for a simulated robot?: A comparison of empathy toward a physical and a simulated robot},
  author={Seo, Stela H and Geiskkovitch, Denise and Nakane, Masayuki and King, Corey and Young, James E},
  booktitle={ACM/IEEE Int. Conference on Human-Robot Interaction},
  pages={125--132},
  year={2015}
}

@article{hupont2019,
  title={Region-based facial representation for real-time Action Units intensity detection across datasets},
  author={Hupont, Isabelle and Chetouani, Mohamed},
  journal={Pattern Analysis and Applications},
  volume={22},
  number={2},
  pages={477--489},
  year={2019},
  publisher={Springer}
}

@inproceedings{HOG,
  title={Histograms of oriented gradients for human detection},
  author={Dalal, Navneet and Triggs, Bill},
  booktitle={IEEE Computer Society Conference on Computer Vision and Pattern Recognition},
  volume={1},
  pages={886--893},
  year={2005}
}

@article{VJ04,
  title={Robust real-time face detection},
  author={Viola, Paul and Jones, Michael J},
  journal={International Journal of Computer Vision},
  volume={57},
  number={2},
  pages={137--154},
  year={2004},
  publisher={Springer}
}

@article{libsvm,
 author = {Chang, Chih-Chung and Lin, Chih-Jen},
 title = {{LIBSVM}: A library for support vector machines},
 journal = {ACM Transactions on Intelligent Systems and Technology},
 volume = {2},
 issue = {3},
 year = {2011},
 pages = {27:1--27:27},
 note =	 {Software available at \url{http://www.csie.ntu.edu.tw/~cjlin/libsvm}}
}

@article{DISFA,
  title={{DISFA}: A spontaneous facial action intensity database},
  author={Mavadati, S Mohammad and Mahoor, Mohammad H and Bartlett, Kevin and Trinh, Philip and Cohn, Jeffrey F},
  journal={IEEE Transactions on Affective Computing},
  volume={4},
  number={2},
  pages={151--160},
  year={2013}
}

@article{sonnby2003emotional,
  title={Emotional empathy as related to mimicry reactions at different levels of information processing},
  author={Sonnby-Borgstr{\"o}m, Marianne and J{\"o}nsson, Peter and Svensson, Owe},
  journal={Journal of Nonverbal behavior},
  volume={27},
  number={1},
  pages={3--23},
  year={2003},
  publisher={Springer}
}

@article{sonnby2002automatic,
  title={Automatic mimicry reactions as related to differences in emotional empathy},
  author={Sonnby--Borgstr{\"o}m, Marianne},
  journal={Scandinavian journal of psychology},
  volume={43},
  number={5},
  pages={433--443},
  year={2002},
  publisher={Wiley Online Library}
}

@article{hofree2018behind,
  title={Behind the robot’s smiles and frowns: In social context, people do not mirror android’s expressions but react to their informational value},
  author={Hofree, Galit and Ruvolo, Paul and Reinert, Audrey and Bartlett, Marian S and Winkielman, Piotr},
  journal={Frontiers in neurorobotics},
  volume={12},
  pages={14},
  year={2018},
  publisher={Frontiers}
}

@article{dimberg2000unconscious,
  title={Unconscious facial reactions to emotional facial expressions},
  author={Dimberg, Ulf and Thunberg, Monika and Elmehed, Kurt},
  journal={Psychological science},
  volume={11},
  number={1},
  pages={86--89},
  year={2000},
  publisher={SAGE Publications Sage CA: Los Angeles, CA}
}

@article{dimberg1990distinguished,
  title={For distinguished early career contribution to psychophysiology: award address, 1988: facial electromyography and emotional reactions},
  author={Dimberg, Ulf},
  journal={psychophysiology},
  volume={27},
  number={5},
  pages={481--494},
  year={1990},
  publisher={Wiley Online Library}
}

@article{dimberg1998rapid,
  title={Rapid facial reactions to emotional facial expressions},
  author={Dimberg, Ulf and Thunberg, Monika},
  journal={Scandinavian journal of psychology},
  volume={39},
  number={1},
  pages={39--45},
  year={1998},
  publisher={Wiley Online Library}
}

@article{kavanagh2016functionality,
  title={The functionality of spontaneous mimicry and its influences on affiliation: An implicit socialization account},
  author={Kavanagh, Liam C and Winkielman, Piotr},
  journal={Frontiers in psychology},
  volume={7},
  pages={458},
  year={2016},
  publisher={Frontiers}
}

@article{winkielman2016mimicry,
  title={Mimicry, emotion, and social context: insights from typical and atypical humans, robots, and androids},
  author={Winkielman, Piotr and Carr, Evan W and Chakrabarti, Bhismadev and Hofree, Galit and Kavanagh, Liam C},
  journal={Emotional mimicry in social context},
  volume={162},
  year={2016},
  publisher={Cambridge University Press}
}

@article{hofree2015observation,
  title={Observation and imitation of actions performed by humans, androids, and robots: an EMG study},
  author={Hofree, Galit and Urgen, Burcu A and Winkielman, Piotr and Saygin, Ayse P},
  journal={Frontiers in human neuroscience},
  volume={9},
  pages={364},
  year={2015},
  publisher={Frontiers}
}

@article{moody2007more,
  title={More than mere mimicry? The influence of emotion on rapid facial reactions to faces.},
  author={Moody, Eric J and McIntosh, Daniel N and Mann, Laura J and Weisser, Kimberly R},
  journal={Emotion},
  volume={7},
  number={2},
  pages={447},
  year={2007},
  publisher={American Psychological Association}
}

@inproceedings{hofree2012you,
  title={Why are you smiling? In a strategic context, people's affective responses reflect the meaning of android's facial expressions},
  author={Hofree, Galit and Ruvolo, Paul and Reinert, Christopher and Bartlett, Marian S and Winkielman, Piotr},
  booktitle={2012 IEEE International Conference on Development and Learning and Epigenetic Robotics (ICDL)},
  pages={1--2},
  year={2012},
  organization={IEEE}
}

@inproceedings{suman2016prior,
  title={Prior behavior impacts human mimicry of robots},
  author={Suman, Apurv and Marvin, Rebecca and Grigore, Elena Corina and Admoni, Henny and Scassellati, Brian},
  booktitle={2016 25th IEEE International Symposium on Robot and Human Interactive Communication (RO-MAN)},
  pages={1057--1062},
  year={2016},
  organization={IEEE}
}

@article{mattheij2015mirror,
  title={Mirror mirror on the wall},
  author={Mattheij, Ruud and Postma-Nilsenov{\'a}, Marie and Postma, Eric},
  journal={Journal of Ambient Intelligence and Smart Environments},
  volume={7},
  number={2},
  pages={121--132},
  year={2015},
  publisher={IOS Press}
}

@article{chartrand2009human,
  title={Human mimicry},
  author={Chartrand, Tanya L and Van Baaren, Rick},
  journal={Advances in experimental social psychology},
  volume={41},
  pages={219--274},
  year={2009},
  publisher={Elsevier}
}

@article{prochazkova2017connecting,
  title={Connecting minds and sharing emotions through mimicry: A neurocognitive model of emotional contagion},
  author={Prochazkova, Eliska and Kret, Mariska E},
  journal={Neuroscience \& Biobehavioral Reviews},
  volume={80},
  pages={99--114},
  year={2017},
  publisher={Elsevier}
}

@article{lishner2008rapid,
  title={Rapid emotional contagion and expressive congruence under strong test conditions},
  author={Lishner, David A and Cooter, Amy B and Zald, David H},
  journal={Journal of Nonverbal Behavior},
  volume={32},
  number={4},
  pages={225--239},
  year={2008},
  publisher={Springer}
}

@inproceedings{mattheij2013vocal,
  title={Vocal and facial imitation of humans interacting with virtual agents},
  author={Mattheij, Ruud and Nilsenova, Marie and Postma, Eric},
  booktitle={2013 Humaine Association Conference on Affective Computing and Intelligent Interaction},
  pages={815--820},
  year={2013},
  organization={IEEE}
}

@article{philip2018rapid,
  title={Rapid Facial Reactions in Response to Facial Expressions of Emotion Displayed by Real Versus Virtual Faces},
  author={Philip, Leonor and Martin, Jean-Claude and Clavel, C{\'e}line},
  journal={i-Perception},
  volume={9},
  number={4},
  pages={2041669518786527},
  year={2018},
  publisher={SAGE Publications Sage UK: London, England}
}

@article{hess1999mimicry,
  title={Mimicry: Facts and fiction},
  author={Hess, Ursula and Philippot, Pierre and Blairy, Sylvie},
  journal={The social context of nonverbal behavior},
  pages={213--241},
  year={1999}
}

@article{chartrand1999chameleon,
  title={The chameleon effect: the perception--behavior link and social interaction.},
  author={Chartrand, Tanya L and Bargh, John A},
  journal={Journal of personality and social psychology},
  volume={76},
  number={6},
  pages={893},
  year={1999},
  publisher={American Psychological Association}
}

@article{bavelas1986show,
  title={" I show how you feel": Motor mimicry as a communicative act.},
  author={Bavelas, Janet B and Black, Alex and Lemery, Charles R and Mullett, Jennifer},
  journal={Journal of personality and social psychology},
  volume={50},
  number={2},
  pages={322},
  year={1986},
  publisher={American Psychological Association}
}

@article{bavelas1986experimental,
  title={Experimental methods for studying “elementary motor mimicry”},
  author={Bavelas, Janet Beavin and Black, Alex and Lemery, Charles R and MacInnis, Scott and Mullett, Jennifer},
  journal={Journal of Nonverbal Behavior},
  volume={10},
  number={2},
  pages={102--119},
  year={1986},
  publisher={Springer}
}

@article{yabar2001dismoi,
  title={Dismoi si vous {\^e}tes intimes, et je te dirais si tu mimes.[Tell me if you’re intimate and I’ll tell you if you’ll mimic] Paper presented at the 24th Annual Meeting of the Soci{\'e}t{\'e} Qu{\'e}b{\'e}coise pour la Recherche en Psychologie},
  author={Yabar, Y and Cheung, N and Hess, U and Rochon, G and Bonneville-H{\'e}bert, N},
  year={2001},
  publisher={October}
}

@article{hatfield1993emotional,
  title={Emotional contagion},
  author={Hatfield, Elaine and Cacioppo, John T and Rapson, Richard L},
  journal={Current directions in psychological science},
  volume={2},
  number={3},
  pages={96--100},
  year={1993},
  publisher={Sage Publications Sage CA: Los Angeles, CA}
}

@article{dimberg1997facial,
  title={Facial reactions: Rapidly evoked emotional responses.},
  author={Dimberg, Ulf},
  journal={Journal of Psychophysiology},
  year={1997},
  publisher={Hogrefe \& Huber Publishers}
}

@article{niedenthal2010simulation,
  title={The Simulation of Smiles (SIMS) model: Embodied simulation and the meaning of facial expression},
  author={Niedenthal, Paula M and Mermillod, Martial and Maringer, Marcus and Hess, Ursula},
  journal={Behavioral and brain sciences},
  volume={33},
  number={6},
  pages={417},
  year={2010},
  publisher={Cambridge University Press}
}

@article{heyes2011automatic,
  title={Automatic imitation.},
  author={Heyes, Cecilia},
  journal={Psychological bulletin},
  volume={137},
  number={3},
  pages={463},
  year={2011},
  publisher={American Psychological Association}
}

@article{buck1980nonverbal,
  title={Nonverbal behavior and the theory of emotion: the facial feedback hypothesis.},
  author={Buck, Ross},
  journal={Journal of Personality and social Psychology},
  volume={38},
  number={5},
  pages={811},
  year={1980},
  publisher={American Psychological Association}
}

@article{niedenthal2007embodying,
  title={Embodying emotion},
  author={Niedenthal, Paula M},
  journal={science},
  volume={316},
  number={5827},
  pages={1002--1005},
  year={2007},
  publisher={American Association for the Advancement of Science}
}

@article{hess1995intensity,
  title={The intensity of facial expression is determined by underlying affective state and social situation.},
  author={Hess, Ursula and Banse, Rainer and Kappas, Arvid},
  journal={Journal of personality and social psychology},
  volume={69},
  number={2},
  pages={280},
  year={1995},
  publisher={American Psychological Association}
}

@article{fischer2012emotional,
  title={Emotional mimicry in social context: the case of disgust and pride},
  author={Fischer, Agneta and Becker, Daniela and Veenstra, Lotte},
  journal={Frontiers in psychology},
  volume={3},
  pages={475},
  year={2012},
  publisher={Frontiers}
}

@article{herrera1998communication,
  title={La communication emotionnelle entre individus de groupes culturels differents [Emotion communication between individuals from different cultural groups]},
  author={Herrera, P and Bourgeois, P and Cheung, N and Hess, U},
  journal={Science et Comportement},
  volume={27},
  pages={S104},
  year={1998}
}

@inproceedings{herrera1998counter,
  title={Counter mimicry effects as a function of racial attitudes},
  author={Herrera, P and Bourgeois, P and Hess, U},
  booktitle={38th Annual Meeting of the Society for Psychophysiological Research, Denver, CO},
  year={1998}
}

@article{hatfield1992primitive,
  title={Primitive emotional contagion},
  author={Hatfield, Elaine and Cacioppo, John T and Rapson, Richard L},
  journal={Review of personality and social psychology},
  volume={14},
  pages={151--177},
  year={1992}
}

@article{epley2007seeing,
  title={On seeing human: a three-factor theory of anthropomorphism.},
  author={Epley, Nicholas and Waytz, Adam and Cacioppo, John T},
  journal={Psychological review},
  volume={114},
  number={4},
  pages={864},
  year={2007},
  publisher={American Psychological Association}
}

@article{waytz2010causes,
  title={Causes and consequences of mind perception},
  author={Waytz, Adam and Gray, Kurt and Epley, Nicholas and Wegner, Daniel M},
  journal={Trends in cognitive sciences},
  volume={14},
  number={8},
  pages={383--388},
  year={2010},
  publisher={Elsevier}
}

@inproceedings{paetzel2018attribution,
  title={The Attribution of Emotional State-How Embodiment Features and Social Traits Affect the Perception of an Artificial Agent},
  author={Paetzel, Maike and Castellano, Ginevra and Varni, Giovanna and Hupont, Isabelle and Chetouani, Mohamed and Peters, Christopher},
  booktitle={2018 27th IEEE International Symposium on Robot and Human Interactive Communication (RO-MAN)},
  pages={495--502},
  year={2018},
  organization={IEEE}
}

@inproceedings{paetzel2017investigating,
  title={Investigating the influence of embodiment on facial mimicry in HRI using computer vision-based measures},
  author={Paetzel, Maike and Varni, Giovanna and Hupont, Isabelle and Chetouani, Mohamed and Peters, Christopher and Castellano, Ginevra},
  booktitle={2017 26th IEEE International Symposium on Robot and Human Interactive Communication (RO-MAN)},
  pages={579--586},
  year={2017},
  organization={IEEE}
}

@article{van2011convergent,
  title={Convergent and divergent responses to emotional displays of ingroup and outgroup.},
  author={Van Der Schalk, Job and Fischer, Agneta and Doosje, Bertjan and Wigboldus, Dani{\"e}l and Hawk, Skyler and Rotteveel, Mark and Hess, Ursula},
  journal={Emotion},
  volume={11},
  number={2},
  pages={286},
  year={2011},
  publisher={American Psychological Association}
}

@article{weyers2009modulation,
  title={Modulation of facial reactions to avatar emotional faces by nonconscious competition priming},
  author={Weyers, Peter and M{\"u}hlberger, Andreas and Kund, Anja and Hess, Ursula and Pauli, Paul},
  journal={Psychophysiology},
  volume={46},
  number={2},
  pages={328--335},
  year={2009},
  publisher={Wiley Online Library}
}

@article{oberman2009slow,
  title={Slow echo: facial EMG evidence for the delay of spontaneous, but not voluntary, emotional mimicry in children with autism spectrum disorders},
  author={Oberman, Lindsay M and Winkielman, Piotr and Ramachandran, Vilayanur S},
  journal={Developmental science},
  volume={12},
  number={4},
  pages={510--520},
  year={2009},
  publisher={Wiley Online Library}
}

@article{niedenthal2001did,
  title={When did her smile drop? Facial mimicry and the influences of emotional state on the detection of change in emotional expression},
  author={Niedenthal, Paula M and Brauer, Markus and Halberstadt, Jamin B and Innes-Ker, {\AA}se H},
  journal={Cognition \& Emotion},
  volume={15},
  number={6},
  pages={853--864},
  year={2001},
  publisher={Taylor \& Francis}
}

@article{hawk2012face,
  title={Face the noise: Embodied responses to nonverbal vocalizations of discrete emotions.},
  author={Hawk, Skyler T and Fischer, Agneta H and Van Kleef, Gerben A},
  journal={Journal of personality and social psychology},
  volume={102},
  number={4},
  pages={796},
  year={2012},
  publisher={American Psychological Association}
}

@article{hess2001facial,
  title={Facial mimicry and emotional contagion to dynamic emotional facial expressions and their influence on decoding accuracy},
  author={Hess, Ursula and Blairy, Sylvie},
  journal={International journal of psychophysiology},
  volume={40},
  number={2},
  pages={129--141},
  year={2001},
  publisher={Elsevier}
}

@article{stel2010mimicry,
  title={Mimicry in social interaction: Benefits for mimickers, mimickees, and their interaction},
  author={Stel, Mari{\"e}lle and Vonk, Roos},
  journal={British Journal of Psychology},
  volume={101},
  number={2},
  pages={311--323},
  year={2010},
  publisher={Wiley Online Library}
}

@article{cheng2003self,
  title={Self-monitoring without awareness: using mimicry as a nonconscious affiliation strategy.},
  author={Cheng, Clara Michelle and Chartrand, Tanya L},
  journal={Journal of personality and social psychology},
  volume={85},
  number={6},
  pages={1170},
  year={2003},
  publisher={American Psychological Association}
}

@article{Martinez2017,
  title={Automatic analysis of facial actions: A survey},
  author={Martinez, Brais and Valstar, Michel F and Jiang, Bihan and Pantic, Maja},
  journal={IEEE transactions on affective computing},
  year={2017},
  publisher={IEEE}
}

@article{ito2004fast,
  title={Fast force-generation dynamics of human articulatory muscles},
  author={Ito, Takayuki and Murano, Emi Z and Gomi, Hiroaki},
  journal={Journal of applied physiology},
  volume={96},
  number={6},
  pages={2318--2324},
  year={2004},
  publisher={American Physiological Society}
}


@article{FASEL2003259,
title = {Automatic facial expression analysis: a survey},
journal = {Pattern Recognition},
volume = {36},
number = {1},
pages = {259-275},
year = {2003},
author = {B. Fasel and Juergen Luettin}
}

@article{varni2017computational,
  title={Computational study of primitive emotional contagion in dyadic interactions},
  author={Varni, Giovanna and Hupont, Isabelle and Clavel, Chloe and Chetouani, Mohamed},
  journal={IEEE Transactions on Affective Computing},
  volume={11},
  number={2},
  pages={258--271},
  year={2017},
  publisher={IEEE}
}

@inproceedings{prepin2013beyond,
  title={Beyond backchannels: co-construction of dyadic stancce by reciprocal reinforcement of smiles between virtual agents.},
  author={Prepin, Ken and Ochs, Magalie and Pelachaud, Catherine},
  booktitle={Proceedings of the Annual Meeting of the Cognitive Science Society},
  volume={35},
  number={35},
  year={2013}
}

@inproceedings{jaques2016understanding,
  title={Understanding and predicting bonding in conversations using thin slices of facial expressions and body language},
  author={Jaques, Natasha and McDuff, Daniel and Kim, Yoo Lim and Picard, Rosalind},
  booktitle={International Conference on Intelligent Virtual Agents},
  pages={64--74},
  year={2016},
  organization={Springer}
}

@article{tickle1990nature,
  title={The nature of rapport and its nonverbal correlates},
  author={Tickle-Degnen, Linda and Rosenthal, Robert},
  journal={Psychological inquiry},
  volume={1},
  number={4},
  pages={285--293},
  year={1990},
  publisher={Taylor \& Francis}
}

@article{gratch2013using,
  title={Using social agents to explore theories of rapport and emotional resonance},
  author={Gratch, Jonathan and Kang, Sin-Hwa and Wang, Ning},
  journal={Social emotions in nature and artifact},
  volume={181},
  pages={181--197},
  year={2013},
  publisher={Oxford University Press Oxford}
}

@inproceedings{wang2009rapport,
  title={Rapport and facial expression},
  author={Wang, Ning and Gratch, Jonathan},
  booktitle={2009 3rd International Conference on Affective Computing and Intelligent Interaction and Workshops},
  pages={1--6},
  year={2009},
  organization={IEEE}
}

@article{bernieri1988coordinated,
  title={Coordinated movement and rapport in teacher-student interactions},
  author={Bernieri, Frank J},
  journal={Journal of Nonverbal behavior},
  volume={12},
  number={2},
  pages={120--138},
  year={1988},
  publisher={Springer}
}

@article{kendon1970movement,
  title={Movement coordination in social interaction: Some examples described},
  author={Kendon, Adam},
  journal={Acta psychologica},
  volume={32},
  pages={101--125},
  year={1970},
  publisher={Elsevier}
}

@article{englis1982conditioning,
  title={Conditioning of counter-empathetic emotional responses},
  author={Englis, Basil G and Vaughan, Katherine B and Lanzetta, John T},
  journal={Journal of Experimental Social Psychology},
  volume={18},
  number={4},
  pages={375--391},
  year={1982},
  publisher={Elsevier}
}

@book{darwin1998expression,
  title={The expression of the emotions in man and animals},
  author={Darwin, Charles and Prodger, Phillip},
  year={1998},
  publisher={Oxford University Press, USA}
}

@book{izard2013human,
  title={Human emotions},
  author={Izard, Carroll E},
  year={2013},
  publisher={Springer Science \& Business Media}
}

@article{tomkins1984affect,
  title={Affect theory},
  author={Tomkins, Silvan S},
  journal={Approaches to emotion},
  volume={163},
  number={163-195},
  year={1984},
  publisher={Hillsdale, NJ}
}

@article{laird1992process,
  title={The process of emotional experience: A self-perception theory.},
  author={Laird, James D and Bresler, Charles},
  year={1992},
  publisher={Sage Publications, Inc}
}

@article{lanzetta1989expectations,
  title={Expectations of cooperation and competition and their effects on observers' vicarious emotional responses.},
  author={Lanzetta, John T and Englis, Basil G},
  journal={Journal of personality and social psychology},
  volume={56},
  number={4},
  pages={543},
  year={1989},
  publisher={American Psychological Association}
}


@article{ekman1983autonomic,
  title={Autonomic nervous system activity distinguishes among emotions},
  author={Ekman, Paul and Levenson, Robert W and Friesen, Wallace V},
  journal={science},
  volume={221},
  number={4616},
  pages={1208--1210},
  year={1983},
  publisher={American Association for the Advancement of Science}
}

@inproceedings{perugia2020role,
  title={On the Role of Personality and Empathy in Human-Human, Human-Agent, and Human-Robot Mimicry},
  author={Perugia, Giulia and Paetzel, Maike and Castellano, Ginevra},
  booktitle={International Conference on Social Robotics},
  pages={120--131},
  year={2020},
  organization={Springer}
}

@article{oosterhof2008functional,
  title={The functional basis of face evaluation},
  author={Oosterhof, Nikolaas N and Todorov, Alexander},
  journal={Proceedings of the National Academy of Sciences},
  volume={105},
  number={32},
  pages={11087--11092},
  year={2008},
  publisher={National Acad Sciences}
}

@inproceedings{calvo2020effects,
  title={The Effects of Robot’s Facial Expressions on Children’s First Impressions of Trustworthiness},
  author={Calvo-Barajas, Natalia and Perugia, Giulia and Castellano, Ginevra},
  booktitle={2020 29th IEEE International Conference on Robot and Human Interactive Communication (RO-MAN)},
  pages={165--171},
  year={2020},
  organization={IEEE}
}

@book{ekman1978facial,
  title={Facial action coding system: Investigator's guide},
  author={Ekman, Paul and Friesen, Wallace V and Hager, Joseph C},
  year={1978},
  publisher={Consulting Psychologists Press}
}

@article{mcintosh2006social,
  title={When the social mirror breaks: deficits in automatic, but not voluntary, mimicry of emotional facial expressions in autism},
  author={McIntosh, Daniel N and Reichmann-Decker, Aimee and Winkielman, Piotr and Wilbarger, Julia L},
  journal={Developmental science},
  volume={9},
  number={3},
  pages={295--302},
  year={2006},
  publisher={Wiley Online Library}
}

@article{hess2014emotional,
  title={Emotional mimicry: Why and when we mimic emotions},
  author={Hess, Ursula and Fischer, Agneta},
  journal={Social and personality psychology compass},
  volume={8},
  number={2},
  pages={45--57},
  year={2014},
  publisher={Wiley Online Library}
}

@article{perugia2021ICanSeeIt,
title={I Can See It in Your Eyes: Gaze as an Implicit Cue of Uncanniness and Task Performance in Repeated Interactions With Robots},      
author={Perugia, Giulia and Paetzel-Prüsmann, Maike and Alanenpää, Madelene and Castellano, Ginevra},
journal={Frontiers in Robotics and AI},      
volume={8},      
pages={78},     
year={2021}
}

@inproceedings{paetzel2020persistence,
  title={The persistence of first impressions: The effect of repeated interactions on the perception of a social robot},
  author={Paetzel, Maike and Perugia, Giulia and Castellano, Ginevra},
  booktitle={Proceedings of the 2020 ACM/IEEE International Conference on Human-Robot Interaction},
  pages={73--82},
  year={2020}
}

@article{paetzel2021influence,
  title={The Influence of robot personality on the development of uncanny feelings},
  author={Paetzel-Pr{\"u}smann, Maike and Perugia, Giulia and Castellano, Ginevra},
  journal={Computers in Human Behavior},
  volume={120},
  pages={106756},
  year={2021},
  publisher={Elsevier}
}

@inproceedings{hoegen2018impact,
  title={The impact of agent facial mimicry on social behavior in a prisoner's dilemma},
  author={Hoegen, Rens and Van Der Schalk, Job and Lucas, Gale and Gratch, Jonathan},
  booktitle={Proceedings of the 18th International Conference on Intelligent Virtual Agents},
  pages={275--280},
  year={2018}
}

@article{numata2020achieving,
  title={Achieving affective human--virtual agent communication by enabling virtual agents to imitate positive expressions},
  author={Numata, Takashi and Sato, Hiroki and Asa, Yasuhiro and Koike, Takahiko and Miyata, Kohei and Nakagawa, Eri and Sumiya, Motofumi and Sadato, Norihiro},
  journal={Scientific reports},
  volume={10},
  number={1},
  pages={1--11},
  year={2020},
  publisher={Nature Publishing Group}
}

@article{riek2010my,
  title={When my robot smiles at me: Enabling human-robot rapport via real-time head gesture mimicry},
  author={Riek, Laurel D and Paul, Philip C and Robinson, Peter},
  journal={Journal on Multimodal User Interfaces},
  volume={3},
  number={1},
  pages={99--108},
  year={2010},
  publisher={Springer}
}

@article{perugia2020engage,
  title={ENGAGE-DEM: a model of engagement of people with dementia},
  author={Perugia, Giulia and D{\'\i}az-Boladeras, Marta and Catal{\`a}-Mallofr{\'e}, Andreu and Barakova, Emilia I and Rauterberg, Matthias},
  journal={IEEE Transactions on Affective Computing},
  year={2020},
  publisher={IEEE}
}

@inproceedings{chung2018your,
  title={“How was Your Stay?”: Exploring the Use of Robots for Gathering Customer Feedback in the Hospitality Industry},
  author={Chung, Michael Jae-Yoon and Cakmak, Maya},
  booktitle={2018 27th IEEE International Symposium on Robot and Human Interactive Communication (RO-MAN)},
  pages={947--954},
  year={2018},
  organization={IEEE}
}
